"From remembering to shaping": Narrating Shared Experiences by Co-Designing Cultural Heritage Artifacts in Collaborative VR

The ways people remember and recall places reveal an invisible aspect of cultural heritage (CH), reflecting how individuals and communities relate to these places. Heritage is communal, emerging through collaboratively constructed narratives rather than individual records. To probe how people may share collective memories, we designed an immersive two-person workflow for collaboratively co-designing 3D artifacts and environments in virtual heritage locations, using Generative AI (GenAI) to instantiate these intangible memories. Observations of the co-creation process revealed that participants merged prompts and model placements when negotiating different perspectives. They used spatial operations to compose scenes, and also to express personal and embodied experiences of CH. When GenAI failed to meet their needs, participants engaged in creative appropriation, re-purposing unsatisfactory generated objects as sources of design inspiration to further shared narratives. While GenAI may have a homogenizing effect on CH expression, this work shows how people may overcome limitations in immersive collaborative workflows.

==> mainacm.tex <==
\newcommand{\removed}[1]{{\color{red} \sout{#1}}}
\newcommand{\replace}[2]{\textcolor{red}{\sout{#1}}\textcolor{blue}{#2}}
\newcommand{\added}[1]{{\color{blue} #1}}

==> sections/CHI_version_old_/01-Intro.tex <==
Cultural heritage (CH) is more than monuments or archives. It also lives in the way people remember everyday places, imagine the future, and negotiate shared meaning, which is an invisible yet vital part of CH \cite{presentisinthefuture}. This aspect of an "invisible heritage" is fundamentally communal \cite{He2025IRecallthePast, Fu2024BeingEroded, giaccardi2012heritage}. It is composed of personal memories and lived experiences that are fragmented across individuals but can manifest collectively through storytelling and negotiation \cite{presentisinthefuture}. These narratives capture the affective and relational ties that connect people to places and are rarely part of any official documentation \cite{jones2017wrestling, presentisinthefuture}.

Despite their significance, conventional heritage approaches often privilege an Authorized Heritage Discourse (AHD) \cite{tsenova2020unauthorised}, emphasizing official histories while marginalizing the unofficial memories, emotions, and local stories that remain vital to cultural identity \cite{han2014heritage, lu2023photovoice, tsenova2023locistories}. Although communities and repeat visitors carry rich experiential knowledge \cite{clarke2018familiar, clarke2021repeat}, they frequently lack accessible means to articulate, visualize, and negotiate these perspectives together. The challenge, therefore, lies not only in preservation but in creating mechanisms for communities to collaboratively author and share plural heritage narratives.

Immersive technologies such as VR and AR have been widely explored for reconstructing cultural heritage sites and enhancing public engagement \cite{bozzelli2019arkaevision,innocente2023immersiveXRframework}. These systems often succeed in providing visually compelling and immersive experiences, yet most are designed around expert-led curation or single-user interaction. As a result, participants are frequently positioned as viewers of pre-defined stories rather than active co-creators of heritage meaning. Even in interactive applications, engagement tends to focus on individual exploration rather than collaborative construction. \cite{innocente2023immersiveXRframework,ShinandWoo2023HowSpaceIsTold} Critically, the spatial potential of VR, that is, the ability for participants to manipulate, reposition, and adapt virtual objects together, has rarely been examined as a medium for collaborative heritage-making. This gap is particularly important because spatial action can serve as a form of negotiation and meaning-making that complements, and at times substitutes, verbal discussion\cite{chang2017evaluatingtheeffectoftangiblevr}. The lack of attention towards this potential motivates our third research question, which specifically examines the role of spatial interaction in shaping collaborative cultural narratives.

To address this gap, we designed an immersive two-person workflow for collaboratively co-constructing cultural memories. In our study, pairs of participants entered a shared VR space with GenAI assistance to visualize and build their memories of urban spaces. Participants verbally described their ideas, which were transcribed and used to generate 3D models. They could then directly manipulate these models-moving, rotating, and combining them-within the shared immersive environment. This setup allowed us to observe how communal heritage narratives are formed through dialogue, negotiation, and spatial action.

Our study is guided by three research questions:

RQ1: How do people collaboratively construct AI-generated cultural heritage visuals in immersive space?

RQ2: How do human-human-GenAI collaborations negotiate differences and resolve challenges?

RQ3: How do spatial manipulations shape the collaborative cultural narrative and the imagination of future cultural spaces?

The study revealed several patterns in collaborative practice. Participants not only merged prompts to reconcile divergence, but often relied on embodied spatial operations, such as repositioning or merging generated objects to co-create cultural scenes, which in some cases reduced the need for verbal negotiation. When generative AI produced unexpected or unsatisfactory outputs, these were not always discarded; instead, participants often reinterpreted them as creative resources, adapting them into new elements of the shared scene (for example, transforming an unintended building into a sculpture). These observations highlight a dynamic interplay between verbal negotiation, direct spatial action, and the creative re-purposing of AI-generated artifacts.

This study contributes an empirical account of how cultural heritage can be represented as a dynamic, immersive co-construction process. By combining generative AI in a collaborative VR environment, we show how people can visualize memories, negotiate perspectives, and creatively reinterpret AI outputs within immersive cultural scenes. Our findings highlight that, together with GenAI, immersive space is not merely a visualization tool but could be a platform for collaborative storytelling. This work advances the understanding of human-human-GenAI collaboration by showing how spatial interaction and generative tools can be combined to support communal ways of authoring and shaping cultural heritage.

==> sections/CHI_version_old_/03-Methods.tex <==
Our study investigates how immersive VR environments, combined with generative AI, can support collaborative reconstruction of cultural heritage spaces from multiple perspectives. In pairs, participants co-created a 3D street scene representing their impressions of Shanghai’s central district, placing AI-generated models directly into a shared VR environment.
\begin{figure} [htp]
 \centering
 \includegraphics[width=1\linewidth]{figures/3-setup.png}
 \caption{An illustration of the study setup. Two participants, each wearing a VR headset, collaboratively interacted with AI-generated 3D models in a shared virtual space. A researcher, external to the VR environment, facilitated the process and recorded data.}
 \Description{An illustration of the study setup. Two participants, each wearing a VR headset, collaboratively interacted with AI-generated 3D models in a shared virtual space. A researcher, external to the VR environment, facilitated the process and recorded data.}
 \label{fig:3-setup}
\end{figure}

\subsection{Participants} 

We recruited 18 participants (9 pairs) through social media outreach, personal contacts, and participant referrals. Participants included both male and female individuals, aged 20-40, from diverse professional backgrounds such as software development, design, law, marketing, and content creation (see demographic figure\ref{Demographic}). We intentionally recruited from diverse fields to capture a broad range of non-expert cultural memories and collaborative styles. The recruited pairs included both acquaintances and strangers to observe a wider range of interaction patterns: six pairs were friends or colleagues, while the remaining three pairs were unacquainted prior to the study. Most participants were novices in VR and generative AI: two had prior VR experience, several had tried conversational AI tools, and a few had limited experience with text-to-image generation. All participants provided informed consent before participation. 
 
All participants provided informed consent before participation. Demographic and background information, including AI/VR experience, cultural heritage familiarity, and collaboration preferences, was collected through a pre-study questionnaire. To ensure participants had a personal connection to the study context, we specifically recruited individuals who had either lived in or visited Shanghai, ensuring they possessed a foundational familiarity with the city. While the sample size (N=18) is not intended for statistical generalization, it is appropriate for an in-depth qualitative exploration of the rich and nuanced collaborative dynamics that are the focus of this study. As our study context is set in Shanghai, we deliberately sought participants who have lived in or visited Shanghai to ensure they have an impression of the city.

\begin{figure}[htp]
 \centering
 \includegraphics[width=1\linewidth]{figures/3.Demographic.png}
 \caption{Demographic table}\label{Demographic}
 \Description{Demographic table}
\end{figure}

\subsection{Study Context}

We situated our study within the cultural context of Shanghai, a global metropolis characterized by its complex history and multi-layered urban memory. One of the city's key cultural identities, the Haipai style \cite{greesnpan2014shanghai}, is a distinctive architectural and cultural style renowned for its fusion of Eastern and Western elements. This provides a rich ground for examining how collective memory is formed and negotiated. 

\subsection{Procedure}

Participants were co-located in the same physical space to foster natural conversation and allow for the observation of non-verbal cues (e.g., gestures, laughter), providing a richer dataset than remote collaboration. The VR environment they shared contained a simplified 3D base map of central Shanghai, providing only geographic references to avoid biasing creative decisions.

The session for each pair was 120 minutes, structured as follows:
\begin{itemize}

\item Training (20 mins): Participants were familiarized with the VR controls and our system through a brief demonstration with example prompts.
\item Collaborative Creation (80 mins): The core task was open-ended: “Construct a street in Shanghai’s central district as you imagine it.” Participants engaged in iterative cycles of generation, placement, and discussion with no restrictions on style or strategy.
\item Semi-structured Interview (20 mins): A post-task interview covered themes of immersion, collaboration, and their experience with the AI.
\end{itemize}

\begin{figure}[htp]
 \centering
 \includegraphics[width=1\linewidth]{figures/3.4-System Design.png}
 \caption{System design and workflow} 
 \Description{System workflow}
 \label{fig:system}
\end{figure}

\subsection{System Design}

We used Meta Quest 3 headsets to host a shared VR environment built on Arkio, a commercial spatial design platform. This platform enabled participants to collaboratively place, resize, and manipulate 3D models using standard VR controllers and provided key environmental controls like custom day-night cycling with dynamic lighting.

A researcher-operated software, GenSH, was developed to assist the use of GenAI models. This ensured accurate prompt delivery, maintained immersion, and avoided interruptions to participants’ creative flow in the immersive space. This avoided typing within the VR interface, which is rather inefficient and may compromise the immersive experience. GenSH provides one-click functions to generate 2D images or 3D models from participant-provided prompts. The AI-generated 3D models could then be imported into the shared VR scene for participants to use and edit.

To maintain immersion and creative flow, we designed a researcher-operated interface, GenSH. This allowed a researcher to accurately transcribe and submit participants' verbal prompts to the AI models, avoiding the need for inefficient in-VR typing, ensuring participants’ creative flow in the immersive space. The AI-generated 3D models were then imported into the shared VR scene for participants to use and edit.

The primary workflow used text-to-image-to-3D generation, and our generative backend employed two models: FLUX.1-dev text-to-image model \cite{flux2024} developed by Black Forest Labs (BFL) and deployed on LibLib platform, and Hunyuan3D \cite{hunyuan3d22025tencent} image-to-3D model by Tencent deployed on Tencent Cloud. Both models were connected via the provided API interfaces that were integrated into our GenSH software for faster generation time. Flux was selected for its high-fidelity images generated from natural language descriptions, while Hunyuan was chosen for its High-precision and stable model generation. 

To address the base models' limited understanding of local architecture and to investigate how culturally-customized AI models affect co-creation, we also trained a custom LoRA model on the Haipai (Shanghai local architecture style) architecture, using a dataset of 312 images of Shanghai buildings trained over 11,000 steps. This model could be applied upon participants' request. In our study design, this custom model was not treated as a formal experimental condition for comparison. Instead, it was provided as an optional tool to empower participants and overcome the known limitations of the base model. Participants were informed that they could request to use this specialized model at any point, particularly if they felt the standard model failed to capture the specific architectural style they envisioned.

To lower the technical barrier and ensure generation quality, the GenSH interface provided preset keywords (e.g., "white background", "45-degree orthogonal view") that could be appended to participants' prompts. Participants were informed that they could adjust or remove these keywords at any time. Similarly, if participants chose to use the Haipai LoRA model, the trigger word "Shanghai building" was appended for the LoRA activation. These preset options were designed to minimize user confusion about the technical process.

\subsection{Data Collection and Analysis}

We collect our data from multiple perspectives:
\begin{itemize}

\item VR environment recording (screen capture of the shared scene).
\item Audio recording of all verbal exchanges.
\item System logs of AI generations, including timestamps and prompts.
\item Photographic and video documentation of the physical session.
\item Researcher observation notes taken in real time.
\end{itemize}

Semi-structured interviews after the task covered immersion, spatial expression, collaboration, AI interaction, and overall impressions. We analyzed the data using reflexive Thematic Analysis \cite{Braun2006}. Interview analysis focused on participants’ reflections on immersion, collaboration, and their perception of AI’s role. Observation analysis coded non-verbal coordination, spatial manipulations, and physical-virtual interactions, not always verbalized. Content analysis systematically categorized all AI-generated 3D models by style (e.g., haipai, modern, hybrid). A table is provided in the appendix.

\subsection{Ethics}

Our research protocol was approved by the university's institutional review board (IRB). Before the study began, all participants provided written informed consent. We informed each person that their participation was voluntary and that they could stop the experiment at any time. To minimize discomfort from using the VR equipment, we instructed participants to report any feelings of nausea or unease immediately. If a participant reported discomfort, they were offered a break or the option to end their participation. In addition, VR devices will be disinfected after each use. All the experiment data was anonymized during transcription and securely stored for academic research use only. 

==> sections/CHI_version_old_/04-Results.tex <==
\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{figures/4.0 summary.png}
    \caption{Screenshots of participants' first-person perspective, the process of creating and editing the generated model in space, and the streets that participants create in VR with GenAI.}
    \Description{Screenshots of participants' first-person perspective, the process of creating and editing the generated model in space, and the streets that participants create in VR with GenAI.}
    \label{fig:summary}
\end{figure}

\subsection{Process of Co-Constructing Shared Memories with GenAI in VR}
\subsubsection{Creating Shared Memories with AI-Generated Objects} 

In our multi-user VR environment, we observed participants using AI-generated 3D objects to visualize their personal and collective memories. One participant's generated object could lead their partner to recall and describe additional details. For example, when P3 generated a simple breakfast shop, P4 immediately recalled a specific detail: "The breakfast shop I remember always had a big steamer at the entrance, steaming hot! We have to add that, it's the soul of the place." They then collaboratively refined the prompt to include this detail. In the post-study interview, P4 reflected that the final scene felt "richer and more detailed than what I could have imagined alone." (figure \ref{fig:breakfast})

\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{figures/4.1.1-breakfast-shop.png}
    \caption{P3's initial generation of a breakfast shop (left) prompted P4 to recall a specific memory of a steamer at the entrance. They then collaborated to add this detail (right), creating a richer, shared scene.}
    \Description{P3's initial generation of a breakfast shop (left) prompted P4 to recall a specific memory of a steamer at the entrance. They then collaborated to add this detail (right), creating a richer, shared scene.}
    \label{fig:breakfast}
\end{figure}

When participants chose to use the custom LoRA model, we observed that the generated content exhibited a stronger Shanghai architectural style. This reduced their need to elaborate on every architectural detail in their prompts. For instance, P17 and P18 initially used the general Flux model and were disappointed, with P17 commenting, "This doesn't look like Shanghai." They then switched to the LoRA model. P18 provided a simple prompt: "Help me generate a red restaurant." The system generated a two-story building with a retro Shanghai style, which met their expectations. They continued to build upon this output, adding more specific details in subsequent prompts. After building out the scene, P18 stated that they "felt as if we had been transported back to that street." (figure \ref{fig:loraprompt})

\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{figures/4.1.1-LoRA-and-Prompts.png}
    \caption{The fine-tuned LoRA model streamlined the creative process. Participants could use simpler prompts (e.g., "a red restaurant") to generate culturally specific architecture, which then served as a foundation for adding more detailed prompts.}
    \Description{The fine-tuned LoRA model streamlined the creative process. Participants could use simpler prompts (e.g., "a red restaurant") to generate culturally specific architecture, which then served as a foundation for adding more detailed prompts.}
    \label{fig:loraprompt}
\end{figure}

\subsubsection{Negotiating by Directly Manipulating Objects in 3D Space}  

We observed that participants frequently used direct manipulation of 3D models to resolve spatial disagreements, often bypassing verbal discussion. In one instance, as in figure \ref{fig:moveaction}, P5 verbally noted that "these two buildings are too close to each other." In response, P6 physically grabbed the models and moved them apart. P5 then replied, "It is better now," and the pair moved to the next task. In another case, P7 and P8 recreated a narrow street from memory. After switching to a first-person perspective to walk through it, P7 remarked, "This feels authentic... But it's too oppressive to walk in." In response, P8 immediately grabbed the building models and dragged them apart to widen the street. After observing the change, P7 asked, "So, can we 'repair' this memory? We have the power now to create and make it better," and proposed designing a plaza. The pair subsequently began discussing new design elements for the widened space. Later in the session, P8 reflected on this change: "Look how interesting our goal has changed after widening the street. We wanted a narrow street, but now we have an avenue."

\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{figures/4.1.2-move-action.png}
    \caption{An example of "action as dialogue." In response to the verbal comment that a street felt "too oppressive," a participant uses direct manipulation to physically drag the buildings apart, immediately resolving the issue and opening up a new design possibility.}
    \Description{The fine-tuned LoRA model streamlined the creative process. Participants could use simpler prompts (e.g., "a red restaurant") to generate culturally specific architecture, which then served as a foundation for adding more detailed prompts.}
    \label{fig:moveaction}
\end{figure}

\subsubsection{Creating and Negotiating from Different VR Perspectives}  

Participants strategically switched between perspectives to manage different collaborative tasks. The god's-eye view was used for macro-level planning and division of labor. For instance, from above the virtual Huangpu River, P9 and P10 decided: "I'll fill the west bank with old buildings," and "I'll take the east bank to build the Lujiazui."

Conversely, the first-person perspective was critical for evaluating aesthetic and affective qualities. Standing on a rooftop of a generated building, P5 remarked, "This feels like standing in Pudong... Now I can look down from any building's top," an experience that triggered personal memories. P5 then invited the partner to share this perspective, creating a moment of shared experience. Later, standing at human scale in front of their co-created coffee shop, they affirmed the scene's authenticity: "This is the feeling! This feels exactly like Shanghai." (figure \ref{fig:perspective})

\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{figures/4.1.3-different-perspective.png}
    \caption{Participants strategically switched between perspectives.}
    \Description{Participants strategically switched between perspectives.}
    \label{fig:perspective}
\end{figure}

\subsubsection{Developing a Modular Building Method of Generated Models} 

During the experiment, we observed several participants developing a modular building method, assembling structures from AI-generated components in a process similar to using Lego blocks.

P13 and P14 first generated a featureless exterior wall from their memory. They then generated separate architectural details, such as Chinese-style tiled roofs, doors, and windows. Using the system's free placement and reshaping tools, they then combined these components to assemble a complete building. This combination was not always planned; in another case, after moving and testing, P11 and P12 combined two unsatisfied generated objects into one new building, which would be discussed further in section 4.3.4.(figure \ref{fig:modular})

Later, they reflected on this method. One participant stated that it "can restore the geometric relationship of the building in my memory," while another noted that it "gives me more control... than directly entrusting the generation of the entire building to AI."

\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{figures/4.1.4-Modular-building.png}
    \caption{Participants developed a modular, "Lego-like" building strategy. They generated individual architectural components, such as walls, roofs, and windows, then used the system's manipulation tools to assemble them into a complete structure.}
    \Description{Participants developed a modular, "Lego-like" building strategy. They generated individual architectural components, such as walls, roofs, and windows, then used the system's manipulation tools to assemble them into a complete structure.}
    \label{fig:modular}
\end{figure}

\subsection{Challenges of Collaboration: Negotiating Differences Between Participants}   
\subsubsection{Using Generated Models to Negotiate Different Memories}  

When partners had different levels of knowledge about the location, the generated 3D models helped them share information. In one pair, this disparity was pronounced: one participant (P16) primarily associated Shanghai with modern skyscrapers, while the other (P15) possessed deeper knowledge of its historical architectural layers. (figure \ref{fig:gap})

To bridge this gap, P15 generated a 3D model of a building in the style of the former Shanghai French Concession area(1849-1943). The 3D model became a shared object they could both see and discuss, turning an abstract description into something concrete. P15 then invited P16 to walk around and through the model together, using the embodied VR space to point out specific features like the roof shape and windows while explaining their cultural significance. This spatial, experiential demonstration was decisive. P16 later reflected: "She kept describing the 'French Concession style,' but I couldn't picture it... When she generated that model and I could walk around it, it was like he opened a door and let me walk directly into her memory." For P15, the model finally provided the means to articulate her vision: "I could finally say, 'See? This is what I was talking about.'" The 3D model allowed the knowledgeable participant to show, rather than just tell, what they meant. This allowed them to move past a limited understanding and learn from each other.

\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{figures/4.2 french concession.png}
    \caption{3D models serving as a cognitive bridge. To explain the abstract concept of "French Concession style" to the partner, P15 generated a representative building. By inviting P16 to walk through the shared model, she transformed an abstract idea into a tangible, experiential lesson.}
    \Description{3D models serving as a cognitive bridge. To explain the abstract concept of "French Concession style" to the partner, P15 generated a representative building. By inviting P16 to walk through the shared model, she transformed an abstract idea into a tangible, experiential lesson.}
    \label{fig:gap}
\end{figure}

\subsubsection{Negotiating Different Cultural Preferences} 

Another example involved cultural associations derived from popular media. P11 initially wanted to build scenes inspired by a television drama, while P12 wanted a film scene. Both the drama and the film show the old part of Shanghai, especially when it comes to setting up the urban scenes, but they have contrasting visual art styles. The TV drama evokes the ambition and prosperity of 1990s Shanghai, and the other film describes a 1940s Shanghai, which is associated with darker pre-liberation themes. To resolve this issue, the pair first generated two rough scenes that reflect each style. After virtually walking through the two contrasting scenes, one participant noted that the scene inspired by the film felt “too narrow and gloomy” from a first-person perspective. Following this embodied comparison, they decided together to adopt the aesthetic of the TV drama. They stated that this style better matched their shared goal of creating what they described as a "vibrant and forward-looking" representation of Shanghai.

\subsection{Challenges of Representation: Reconciling with GenAI Outcomes}
\subsubsection{Unexpected Generation} 

The GenAI sometimes generated content beyond the use of prompts. Within the three-dimensional VR environment, participants often entered new spaces and incorporated new and unplanned designs into the spaces.

For example, when a pair generated a street-corner coffee shop. The AI not only created the building's exterior but also generated an interior space, which was not requested. This surprise led participants to discuss how to decorate the interior. P1 exclaimed, "Wow, I didn't ask for an interior! Quick, let's go in and see...". P2 replied: "It's too empty here, we need to add some bar stools and pendant lights." The pair then proceeded to generate the decorations and began furnishing the interior together.

In another case of generating an office building (Pair 3), GenAl added commercial space on the ground floor, even including a small plaza and green beds around it. Participants found this street scene very similar to their memory of Shanghai street and started to expand the street based on this extra space, such as adding local elements like yellow and green shared bicycles. (figure \ref{fig:interior})

\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{figures/4.3.1-interior-space.png}
    \caption{Creative adoption of unexpected AI outputs. When the AI generated an unprompted interior space for a coffee shop, participants did not view it as an error but immediately began collaborating on how to furnish and decorate the new space.}
    \Description{Creative adoption of unexpected AI outputs. When the AI generated an unprompted interior space for a coffee shop, participants did not view it as an error but immediately began collaborating on how to furnish and decorate the new space.}
    \label{fig:interior}
\end{figure}

\subsubsection{Generating for Day and Night}
We observed that the ability to set the virtual time of day and change of lighting prompted participants to generate time-specific elements. For example, in a nighttime setting, P13 generated street lamps. Additionally, P15 and P16 conceived that “a Shanghai street at night should present a vivid and bustling atmosphere filled with colorful lights”. Consequently, they generated architectures such as theaters and restaurants adorned with neon and warm lights.

\subsubsection{Hybrid Generation} 

When participants had conflicting style preferences, we observed instances where they used the AI to generate a hybrid compromise. In these cases, participants described the AI's output as "inspiration" that blended both of their ideas. It is neither entirely aligned with one party's requirements nor simply a summation of them, but a result that was described by participants as "inspiration that blended both ideas”.

Hybrid generation was clearly illustrated by P17 and P18, who disagreed on what represented "authentic" Shanghai: one argued for the old, vibrant alleyways ("longtang"), while the other argued for a modern, international metropolis. Unable to agree on their views, they wrote a contrast prompt: "A modern high-rise building with some traditional Chinese elements." The AI's output, a building that seamlessly blended modern and vintage stylistic elements, was accepted by both parties as a successful and satisfying compromise. They placed this building at the entrance to their alleyway and decided to use this hybrid style as a template for further co-creation. They reflected that the AI's solution “captured and represented Shanghai's embracing spirit”. (figure \ref{fig:hybrid})

\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{figures/4.3.3-hybrid-outcom.png}
    \caption{The AI acting as a mediator to resolve conflict. When P17 and P18 disagreed on architectural styles, they co-authored a hybrid prompt. The AI's output, which successfully blended both of their visions, was accepted as a satisfying compromise.}
    \Description{The AI acting as a mediator to resolve conflict. When P17 and P18 disagreed on architectural styles, they co-authored a hybrid prompt. The AI's output, which successfully blended both of their visions, was accepted as a satisfying compromise.}
    \label{fig:hybrid}
\end{figure}




\subsubsection{Collectively Responding to GenAI’s Shortcomings} 

When GenAI outputs failed to meet expectations, participants did not see it as a dead end. Instead, they collaboratively developed and employed three typical strategies to adapt, repurpose, or work around these limitations, demonstrating their ability to maintain creativity despite AI limitations.

\textit{Repurposing "Failed" Generated Models} One strategy was to find a new use for an object that the AI generated incorrectly. A clear instance of this occurred when a pair attempted to generate a specific architectural feature ("a building with side stairs and a car ramp"). The AI instead produced a structure with illogical columns and a spiral staircase. Rather than discarding it, the pair physically rotated the model, discussed its new potential, and collectively re-narrated it as a "futuristic city installation." They then decided to place it in their street as a central artistic feature. As P10 concluded: "Alright, clearly a car cannot drive up it. But look at it... It doesn't look like a building, more like an installation. ” P9 added: “Let's make it a sculpture then.” In another example, P8 took a model generated by P7, scaled its height, and repurposed it as their virtual city's "Oriental Pearl TV Tower", as seen in figure \ref{fig:tower}.

This strategy was not limited to single objects. As noted earlier (in Section 1.2.3), participants would sometimes regard multiple AI outputs as "components" and combine them to be a new, coherent structure that better matched their intent. This strategy also included unsatisfied outputs. For example, group 6 tried to generate a flower shop, GenAI only returned the front face, without the side and back. They then decided to put this front face onto a gray building, because "the gray building is dull, not like a vibrant Shanghai street that we are picturing.".

\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{figures/4.3.4-repurpose.png}
    \caption{Creative repurposing of a "failed" generation.}
    \Description{Creative repurposing of a "failed" generation.}
    \label{fig:tower}
\end{figure}

\textit{Iterate on successful aspects of failed outputs} A second strategy was to identify one good feature in a failed generation and use it as a starting point for new prompts. Participants would identify a satisfied aspect of a failed output and iterate upon it through subsequent prompts.

For example, P12 requested a "building with a cat-shaped neon sign on the roof." The AI generated only the neon sign, without the building itself. However, the group was satisfied with the visual style of the neon sign. They therefore abandoned the original goal and adopted a new strategy: using "neon style" as the core prompt for future actions, such as generating a "neon style chair." This allowed them to build up a consistent aesthetic atmosphere, despite the AI's initial failure to comprehend the full request. (figure \ref{fig:neon})

\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{figures/4.3.4-neon-cat.png}
    \caption{The AI failed to generate a complete building but successfully created a "cat-shaped neon sign" in a style the participants liked. They then adopted "neon style" as a core creative constraint for subsequent generations.}
     \Description{The AI failed to generate a complete building but successfully created a "cat-shaped neon sign" in a style the participants liked. They then adopted "neon style" as a core creative constraint for subsequent generations.}
    \label{fig:neon}
\end{figure}

\subsubsection{Encountering and Responding to Biased Outputs}

We also observed that without using the custom LoRA, the base GenAI model sometimes generated outputs that participants perceived as stereotypical, as in figure \ref{fig:laracompare}. For instance, when P13 tried to generate "A building with a street lamp that emits warm yellow light... integrating Chinese and Western styles", the model produced a building with elements like "excessively upturned dougong", "lanterns", "overwhelming Chinese red”, and "Chinese horticulture". P13 reacted negatively to this output, commenting: "This is too Western. It looks like a building from the underworld. I don't like this outcome."

\begin{figure}[htp]
    \centering
    \includegraphics[width=1\linewidth]{figures/4.3.5-LoRA.png}
    \caption{The comparison of using and not using custom LoRA.}
    \Description{The comparison of using and not using custom LoRA.}
    \label{fig:laracompare}
\end{figure}

==> sections/CHI_version_old_/05-Discussion.tex <==
\subsection{Beyond Language: Embodied Action as Dialogue}
Research on teams using GenAI established a baseline for language-driven collaboration on 2D screens, where participants primarily negotiated through iterative textual prompts, positioning the AI as an "efficient tool" \cite{han2024teams}. Our study, set in a multi-user immersive 3D environment, revealed a different pattern. While verbal negotiation occurred, we observed that direct physical manipulation often served as a more immediate form of dialogue. For instance, a verbal comment like "these two buildings are too far apart" was frequently answered not with a revised prompt, but with the physical action of moving the models closer. These observations suggest that when AI outputs are tangible artifacts in a shared space, the focus of negotiation can shift from language to action. This points to a spatially embodied paradigm for co-creation, where narrative emerges through physical manipulation \cite{Yang2022TowardsImmersiveCollaborativeSensemaking}.

\subsection{The AI as a Generative Mediator}
The 2D and language-centric methodology in a recent study led to findings that framed the AI as an "efficient tool" \cite{han2024teams}. Our methodology, which embedded AI-generated objects in a shared 3D space, allowed us to observe the AI taking on a more social, mediating role in the human-human creative process. We documented two mediating strategies: participants tasking the AI with generating hybrid compromises to resolve impasses (e.g., accepting its output as a "third voice"), and collaboratively re-narrating its "failures" into new features (e.g., reinterpreting an illogical structure as a "futuristic installation"). In our study, the AI's primary value lay not in efficient task execution, but in generating negotiable artifacts that provoked discussion and facilitated the building of shared meaning between users.

\subsection{From Biased Output to Boundary Object}
Previous work demonstrated a significant risk in single-user AI interactions: users lacking domain knowledge may uncritically accept biased or stereotypical outputs \cite{He2025IRecallthePast}. Our collaborative VR setting revealed a potential mitigation strategy. When a knowledge gap existed between participants, AI-generated models often functioned as "boundary objects" \cite{star1989institutional}. The more knowledgeable participant would use the model as a concrete reference, guiding their partner through it and explaining cultural nuances. This suggests that the risks associated with AI bias can be mediated by social and interactive contexts. The same output that might mislead an individual became a shared reference point for teaching, learning, and building a more nuanced collective understanding.

\subsection{Co-Creation as a Civic Sandbox}
Although our study focused on memory reconstruction, we observed a recurring pattern: the hands-on process of building and manipulating the environment often led participants to shift from discussing the past ("What was here?") to imagining the future ("What could be here?"). This sense of direct control, a known affordance of VR \cite{chang2017evaluatingtheeffectoftangiblevr}, appeared to empower participants to engage in proactive design. This observed shift indicates that such systems could function as "low-risk sandboxes," enabling communities to prototype, visualize, and negotiate future visions for their shared spaces. This potential application in participatory urban planning presents a promising direction for future research.

\subsection{Limitations and Future Work}
\subsubsection{Limitations of Ecological Validity in Virtual Heritage}

Our study was conducted in a controlled VR environment, which, while necessary for the experiment, is not ecologically valid in representing how heritage discussions naturally occur. In the real world, collaborative remembering is closely tied to the surrounding environment. The physical scale of a building, the ambient sounds of a neighborhood, or the texture of a wall are all powerful sensory cues that trigger memories and shape conversation. By conducting the study away from the actual heritage site, participants could not draw on these immediate sensory details as a shared reference for their generative prompts. For example, the way participants pointed to and discussed a digital model on a virtual table is fundamentally different from how they might gesture towards a real building while standing on the street. A study found that in the VR experience of Mogao cave, people could not experience the multi-sensory scenarios of the real caves, including spatial atmosphere, sound, smell, and historical traces. Furthermore, the VR images are "too bright, too fresh and too vivid", which does not match the "mottled and dim" historical sense of the real caves \cite{zhao2021playfulness}. Another empirical study showed that in heritage-related VR, satisfaction is mainly driven by "activity-related authenticity". Although VR is effective at reconstructing scenes, the satisfaction of heritage-related experiences depends more on the authenticity of "situations/activities" \cite{nam2023authenticity}. These findings indicate the ecological validity limitations of VR relative to the real site.

Future work could address this by using Augmented Reality (AR). A follow-up study could involve participants walking through the actual site, with AR used to overlay and manipulate generative AI-generated models directly in the real-world environment. This would allow us to observe how real-world landmarks and the physical presence of other people influence the prompts participants create together.

\subsubsection{Limitations of Group Dynamics}

Our study focused exclusively on pairs, which simplifies the complex social dynamics present in larger groups. The collaborative strategies we observed, such as merging prompts or treating GenAI as a "third voice", are well-suited to one-on-one negotiation. However, these findings may not directly translate to larger groups. For instance, in a group of three or five, new challenges would emerge: how would the group decide whose prompt to submit? How would subgroups form and influence decisions? Would the GenAI's role as a mediator still be effective in a two-vs-one scenario? The tasks of capturing and responding to prompts, managed by a researcher in our study, would also become significantly more complex.

Research on multi-person collaboration with GenAI suggests that as group size increases, behaviors, consensus-seeking strategies, and methods for resolving contradictions become more varied and complex. A study explored a collaborative learning model for three-person groups using GenAI, in which members switched among five modes depending on task context \cite{perifanou2025collaborative}. Examining groups of three or more would help clarify how social structure and interaction shape collaborative remembering. This might lead to more complex social phenomena such as leadership, consensus-building, and turn-taking, as participants jointly decide how to instruct the AI.

Additionally, our study included six pairs of acquaintances and three pairs of strangers. While we observed that acquaintances seemed to communicate more smoothly, the limited sample size prevents us from making firm claims about how these relationships affected collaborative patterns. Differences between acquaintances and strangers, as well as those among various gender combinations, are also worth further exploration.

\subsubsection{The Representational Fidelity of Generative Models}

Our study relied on the current capabilities of GenAI, and the resulting 3D models, while stylistically appropriate, could not fully replicate the realistic details of real-world architecture. We used a fine-tuned LoRA model to ensure the generated buildings aligned with the Haipai architectural style, capturing its core structural and formal elements to some extent. However, the finer details, such as the texture of brickwork, the reflection on a window pane, or the subtle rust on the facade, were often rendered with a degree of abstraction or blurriness. Also, the image-to-3D pipeline introduced issues of geometric fidelity. Because our training photos were often taken from a single angle, the AI could not infer occluded parts of a building, resulting in incomplete models that sometimes contain only a front facade. This limited the participants' ability to explore their memories in 3D space. Moreover, in our VR experiment environment, the missing optimization for the generated model's triangular mesh can cause incomplete display issues. A study found that when GenAI was used for the documentation, protection, and restoration of cultural heritage, the current GenAI models had problems, such as inaccuracy in automatic image classification and limitations in generated image quality \cite{silva2024artificial}. Similarly, another study reports that GenAI output quality depends on the quantity, quality, and diversity of its training data. Limited training data can lead to distortion of 3D models, and current methods cannot fully reproduce the authenticity or perceived 'aura' of original works \cite{spennemann2024generative}. Our participants, in essence, negotiated and co-created with a simplified, somewhat idealized version of their memories rather than with a photorealistic replica.

This gap between the generated representation and physical reality could have influenced the collaborative process. For instance, the lack of fine-grained, realistic detail could have made it easier for participants to merge their differing perspectives, as there were fewer concrete, high-fidelity features to contest. Conversely, it might have also limited the depth of memory recall, as the specific sensory details that often trigger memories were absent \cite{buchanan2007Retrievalofemotionalmemories}.

Future research should empirically investigate how model fidelity and realism affect collaborative memory construction. A comparative study, for example, could contrast the collaborative patterns observed using generative models (like ours) with those observed using high-fidelity, photogrammetry-based digital twins of the same heritage sites. This would help reveal how the level of realism in a shared artifact either constrains or enables the negotiation of collective memory.

\subsubsection{GenAI Model Lacking Specific Cultural understanding}

When generating historical buildings, the general GenAI model has a limited understanding of local architectural terms in Shanghai. During the study, the model failed to generate key elements in the prompt, such as specific architectural styles like "arcade-style buildings" and "Shanghai-style", or local materials like "granitic plaster" and "red brick jointing". The resulting models contained inaccuracies or stylistic errors and did not match what the participants described, and they couldn't precisely follow the real intention of the participants. For instance, the general model couldn't accurately understand the participant's prompt "Shikumen-style" residential buildings. To resolve this issue, we have prepared a LoRA model for participants to choose to use. However, our LoRA only targeted the Haipai style of the specific area, while it did not represent all architectural styles in Shanghai and cover all the ideas of the participants. This indicated that improvements were needed for GenAI models to ensure the accuracy of culturally relevant content.

\subsubsection{Limited Demographic Scope of Participants}
\textit{Lack of Cultural Diversity}
While our participant sample was appropriate for an in-depth qualitative study, its diversity was limited. Most participants were young adults with a shared cultural background and some familiarity with digital technologies. The collaborative patterns and the specific heritage memories we observed appear linked to this specific demographic. 
Shanghai itself is a highly diverse city. We selected Shanghai as the study site. As an international metropolitan and a former colonial city, Shanghai has one of the largest migrant populations in China \cite{wong2005building}. The city brings together residents from various domestic provinces as well as from different countries around the world. This demographic and ethnic diversity provided a diverse narrative perspective for the collective memory and cultural construction of the city. A group with different backgrounds, for example, elderly long-term residents, recent immigrants, or professional architects, would likely construct distinctly different narratives and exhibit different collaborative styles. Their relationship with "Haipai" heritage, and therefore their negotiation process, could be substantially different.

Future studies could deliberately recruit participants with more diverse relationships to the heritage site to explore how different standpoints influence the co-construction of memory. A comparison between the interactions of long-term residents and those of tourists, for example, could provide deeper insights into how collective identity is represented and contested in this process. Future studies could also incorporate a broader range of nationalities and cultural backgrounds, such as pairing Chinese and international participants, to understand cross-cultural collaborative dynamics better.

\textit{Lack of Inter-generational Representation} Although our participants were of different ages, they were mainly adults aged between 20 and 40. The elderly tend to have deeper historical memories, while the younger generation may offer more digital or future-oriented perspectives. The absence of older or much younger participants limits the breadth of the collective memory we captured. Previous studies have revealed differences in narrative styles and memory content between different generations. These differences reflect the dynamics of cultural inheritance \cite{buccitelli2016ve}. A study that organized digital narrative workshops between the elderly and senior primary school students. Has demonstrated the effectiveness of promoting inter-generational relationships and cultural conservation in indigenous communities \cite{freeman2020use}. Especially in rapidly developing cities such as Shanghai, the cities have changed greatly from generation to generation, which leads to significant differences in memory among different generations. 
Future research should incorporate inter-generational dialogue groups to study how memories are jointly constructed across generations, rather than merely collecting stories from different generations in parallel.

\subsection{Design Implications}
\subsubsection{Enhance the GenAI Usage Experience in VR Space}

In our work, the application of GenAI in the VR environment has not been fully integrated. An ideal system should allow users to directly operate GenAI models in the VR environment and edit the generation prompts. However, text input in VR is rather inconvenient; even if a voice recognition solution is adopted, there are significant challenges in terms of translation accuracy, filtering of modal particles, and the convenience of modification. Therefore, in this study, the prompt input was assisted by the experimenters, and the potential of real-time, dynamic co-creation of prompts by participants in the virtual space was not fully explored.

Furthermore, as the GenAI-generated models lack topological optimization of their Triangular Mesh, the resulting polygon count is excessively high, which substantially increases the system's rendering load. When the total number of polygons in a scene becomes too large, issues such as incomplete model display, system lag, and unresponsive interactions frequently occur. These problems indicate that both VR hardware and GenAI systems require further improvements to meet the demands for immersive experiences.

\subsubsection{Enhance GenAI's Generative Ability Regarding Culture-related Elements}

Although we have collected a certain amount of photos of Shanghai's Haipai architecture as the training dataset for LoRA, many of these photos were taken from a single angle, and the back or side facades of the buildings may be obscured, making it impossible to obtain their appearance information. Current image-to-3D models are heavily dependent on the visible information in the input images and have difficulty inferring and completing parts of buildings that were not captured based on prior knowledge \cite{PANG2022102859}, such as the architectural style and symmetry of the back facades and roof structures of “lilong” houses. As a result, the generated 3D models are often partial and incomplete, sometimes generating only the front of the building. Thus, adding more multi-angle perspectives of buildings to the training dataset or enhancing the image-to-3D model's reasoning ability related to cultural elements is warranted.

\subsubsection{Social Practice}

A key finding is that collaborative processes often led participants to start imagining future possibilities for their city. Thus, systems can explicitly facilitate future-oriented tasks, such as by adding prompts or templates that ask users to "design a solution for future tourism noise" or "imagine what this will look like in 50 years under the current climate trend." Positioning these tasks as core elements of the system enhances its effectiveness as a “civic sandbox” for community planning. Finally, the scenes created by users should be easy to share and display, both online and in community spaces, to spark wider public discussion and negotiation.

==> sections/CHI_version_old_/06-Conclusion.tex <==
%202509CHI
This work illustrates a shift from passively remembering cultural heritage to actively co-shaping it in a shared, immersive space. In the virtual environment that we built, participants turned personal memories into tangible AI-generated artifacts. Additionally, negotiation shifted from purely verbal to being spatial, as participants resolved differences by physically moving, combining, and repurposing the generated models. This process transforms a workflow into a "sandbox" for community expression. It also redefines the AI's role: not as a tool for producing answers, but as a mediator that facilitates human collaboration. Designing for this multi-human-AI partnership is a critical direction for future collaborative creative design systems.


